SP3D: Boosting Sparsely-Supervised 3D Object Detection via Accurate Cross-Modal Semantic Prompts

Recently, sparsely-supervised 3D object detection has gained great attention, achieving performance close to fully-supervised 3D objectors while requiring only a few annotated instances. Nevertheless, these methods suffer challenges when accurate labels are extremely absent. In this paper, we propose a boosting strategy, termed SP3D, explicitly utilizing the cross-modal semantic prompts generated from Large Multimodal Models (LMMs) to boost the 3D detector with robust feature discrimination capability under sparse annotation settings. Specifically, we first develop a Confident Points Semantic Transfer (CPST) module that generates accurate cross-modal semantic prompts through boundary-constrained center cluster selection. Based on these accurate semantic prompts, which we treat as seed points, we introduce a Dynamic Cluster Pseudo-label Generation (DCPG) module to yield pseudo-supervision signals from the geometry shape of multi-scale neighbor points. Additionally, we design a Distribution Shape score (DS score) that chooses high-quality supervision signals for the initial training of the 3D detector. Experiments on the KITTI dataset and Waymo Open Dataset (WOD) have validated that SP3D can enhance the performance of sparsely supervised detectors by a large margin under meager labeling conditions. Moreover, we verified SP3D in the zero-shot setting, where its performance exceeded that of the state-of-the-art methods. The code is available at https://github.com/xmuqimingxia/SP3D.

==> FigText/pipeline.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=1\linewidth]{Figs/pipeline.pdf}
   \caption{Illustration of SP3D-assisted sparsely-supervised 3D object detection. (a) LMMs-guide training; (b) Fine-tuning using sparse labels.
}
   \label{fig:pipeline}
\end{figure*}

==> TableText/car_ratio.tex <==
\begin{table}[ht]
\setlength{\tabcolsep}{6pt}
\centering
\begin{tabular}{ccccc}
% \hline
\toprule
\multirow{2}{*}{Anno. Rate} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Car-3D @IoU 0.7} \\ \cline{3-5} 
                                 &                          & Easy    & Mod     & Hard   \\ 
                                 \hline
100\%                            & CenterPoint            & 89.07   & 80.50   & 76.49  \\ 
% \midrule
\hline
\multirow{2}{*}{10\%}            & CoIn                  & 85.95   & 71.80   & 62.64  \\
                                 & + 
 E3D                      & 88.84   & 73.56   & 65.17  \\ 
 % \midrule
 \hline
\multirow{2}{*}{5\%}             & CoIn                      & 81.64   & 67.48   & 58.32  \\
                                 & + E3D                      & 87.52   & 72.42   & 63.87  \\ 
                                 \hline
                                 % \midrule
\multirow{2}{*}{2\%}             & CoIn                      & 72.03   & 54.82   & 43.77  \\
                                 & + E3D                      & 87.44   & 69.24   & 58.61  \\ 
                                 % \midrule
                                 \hline
\multirow{2}{*}{1\%}             & CoIn                    & 70.39   & 51.31   & 41.31  \\
                                 & + E3D                      & 83.79   & 63.16   & 52.50  \\ 
                                 % \midrule
                                 \hline
\multirow{2}{*}{0.5\%}           & CoIn                     & 66.77   & 47.68   & 38.38  \\
                                 & + E3D                      & 80.36   & 59.99   & 49.44  \\ 
                                 % \midrule
                                 \hline
\multirow{2}{*}{0.2\%}           & CoIn                      & 45.47   & 31.20   & 23.52  \\
                                 & + E3D                      & 75.30   & 52.99   & 42.14  \\ 
                                 % \midrule
                                 \hline
\multirow{2}{*}{0.1\%}           & CoIn                     & 6.84    & 4.65    & 3.61   \\
                                 & + E3D                      & 58.57   & 37.41   & 29.88  \\ 
                                 \bottomrule
                                 % \hline
       \end{tabular}
       \caption{Comparison with different annotation rates (10\% $\to$ 0.1\%). We report the results with 40 recall positions, under
0.7 IoU threshold.}
        \label{tab:ablation}
\end{table}

==> TableText/recall_compare.tex <==
\begin{table}[ht]
\setlength{\tabcolsep}{4pt}
\centering

\begin{tabular}{cccc}
\toprule
Recall & @IoU 0.3 & @IoU 0.5 & @IoU 0.7 \\ 
\midrule
CoIn   & 0.67     & 0.63     & 0.46     \\
+ E3D    & 0.84     & 0.79     & 0.61     \\ 
\textit{Improvement}    & 0.17     & 0.16     & 0.15 \\
\bottomrule
\end{tabular}
\caption{The comparison of Recall on different IoU thresholds (0.3, 0.5, 0.7). }
\label{tab:ablation}
\end{table}

==> TableText/zero-shot-sup.tex <==
\begin{table*}[ht]
\setlength{\tabcolsep}{4pt}
\centering

\begin{tabular}{c|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Modality} & \multicolumn{2}{c|}{ Vehicle L2 @$IoU_{0.7}$} & \multicolumn{2}{c|}{ Pedestrian L2 @$IoU_{0.5}$} & \multicolumn{2}{c}{ Cyclist L2 @$IoU_{0.5}$} \\
& Train & Test &  \mathbf{AP} \uparrow  &  \mathbf{APH} \uparrow  &  \mathbf{AP} \uparrow  &  \mathbf{APH} \uparrow  &  \mathbf{AP} \uparrow  &  \mathbf{APH} \uparrow  \\
\hline 
SAM3D & L & L & 19.1 & 13.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
CM3D  & L + C & L &23.7 &17.5 &0.1 &0.1 &2.6 &1.3 \\
 \textbf{E3D (Ours)}  & L + C & L & \textbf{35.0} & \textbf{31.8} & \textbf{15.7} & \textbf{6.7} & \textbf{5.8}& \textbf{4.4} \\

\hline
\end{tabular}
\caption{Comparison with zero-shot methods on the WOD validation set. We report Level-2 mAP and mAPH with IoU thresholds of 0.7, 0.5, and 0.5 for Vehicle, Pedestrian, and Cyclist, respectively.}
\label{tab:zero-shot-sup}
\end{table*}

==> sec/X0_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
